Penrose process in radiating Kerr-Vaidya black holes: efficiency, energy transport, and the viability boundary

We study single-particle Penrose extraction from a rotating black hole whose mass decreases in time, described by the ingoing Kerr-Vaidya metric, imposing exact four-momentum conservation at the decay. We prove that the local efficiency is bounded by the instantaneous Kerr value, through a covariant bound that reduces to the Bardeen-Press-Teukolsky limit at the horizon, and we derive an exact transport law, dE/dtau = -dm/dt (r/Sigma) p_r^2 for fixed spin parameter, by which every timelike geodesic gains energy while the hole loses mass. The net energy gain therefore splits into a local Penrose term and two transport terms, which we compute numerically as functions of spin and mass-loss rate for two mass-loss laws. With fixed spin parameter, extraction is possible only below a critical rate alpha_crit(a) = (M-a)/Delta v, set by the approach of the hole to extremality; with fixed a/m no such boundary exists. The transport law extends to the Kerr-Newman-Vaidya family, and the regime where the dynamics matter is shown to lie far outside astrophysical mass-loss rates.

==> table_budget_v2.tex <==
-- & 0.9 & 0 & 0.900 & 0.000 & 0.055 & 0.000 & 0.055 \\
A & 0.9 & $10^{-4}$ & 0.902 & 0.002 & 0.053 & 0.083 & 0.138 \\
A & 0.9 & $10^{-3}$ & 0.920 & 0.023 & 0.068 & 0.086 & 0.178 \\
A & 0.9 & $10^{-2}$ & 0.947 & 0.021 & 0.088 & 0.000 & 0.110 \\
A & 0.9 & $10^{-1}$ & 0.947 & 0.013 & 0.089 & 0.000 & 0.102 \\
-- & 0.95 & 0 & 0.950 & 0.000 & 0.092 & 0.000 & 0.092 \\
A & 0.95 & $10^{-4}$ & 0.951 & 0.001 & 0.076 & 0.248 & 0.325 \\
A & 0.95 & $10^{-3}$ & 0.970 & 0.028 & 0.125 & 0.132 & 0.285 \\
A & 0.95 & $10^{-2}$ & 0.995 & 0.017 & 0.163 & 0.000 & 0.180 \\
A & 0.95 & $10^{-1}$ & 0.995 & 0.010 & 0.164 & 0.000 & 0.174 \\
-- & 0.99 & 0 & 0.990 & 0.000 & 0.150 & 0.000 & 0.150 \\
A & 0.99 & $10^{-4}$ & 0.993 & 0.010 & 0.165 & 0.061 & 0.236 \\
A & 0.99 & $10^{-3}$ & 0.999 & 0.006 & 0.187 & 0.000 & 0.193 \\
A & 0.99 & $10^{-2}$ & 0.999 & 0.002 & 0.188 & 0.000 & 0.190 \\
A & 0.99 & $10^{-1}$ & 0.999 & 0.002 & 0.188 & 0.000 & 0.190 \\
\midrule
B & 0.9 & $10^{-4}$ & 0.900 & 0.009 & 0.055 & 0.030 & 0.094 \\
B & 0.9 & $10^{-3}$ & 0.900 & 0.016 & 0.055 & 0.023 & 0.094 \\
B & 0.9 & $10^{-2}$ & 0.900 & 0.017 & 0.055 & 0.000 & 0.072 \\
B & 0.9 & $10^{-1}$ & 0.900 & 0.014 & 0.055 & 0.000 & 0.069 \\
B & 0.95 & $10^{-4}$ & 0.950 & 0.005 & 0.091 & 0.041 & 0.136 \\
B & 0.95 & $10^{-3}$ & 0.950 & 0.016 & 0.091 & 0.022 & 0.129 \\
B & 0.95 & $10^{-2}$ & 0.950 & 0.017 & 0.091 & 0.000 & 0.108 \\
B & 0.95 & $10^{-1}$ & 0.950 & 0.014 & 0.091 & 0.000 & 0.105 \\
B & 0.99 & $10^{-4}$ & 0.990 & 0.003 & 0.148 & 0.055 & 0.206 \\
B & 0.99 & $10^{-3}$ & 0.990 & 0.015 & 0.149 & 0.019 & 0.183 \\
B & 0.99 & $10^{-2}$ & 0.990 & 0.017 & 0.148 & 0.000 & 0.165 \\
B & 0.99 & $10^{-1}$ & 0.990 & 0.013 & 0.149 & 0.000 & 0.162 \\

